A Weakness Measure for GR(1) Formulae

In spite of the theoretical and algorithmic developments for system synthesis in recent years, little effort has been dedicated to quantifying the quality of the specifications used for synthesis. When dealing with unrealizable specifications, finding the weakest environment assumptions that would ensure realizability is typically a desirable property; in such context the weakness of the assumptions is a major quality parameter. The question of whether one assumption is weaker than another is commonly interpreted using implication or, equivalently, language inclusion. However, this interpretation does not provide any further insight into the weakness of assumptions when implication does not hold. To our knowledge, the only measure that is capable of comparing two formulae in this case is entropy, but even it fails to provide a sufficiently refined notion of weakness in case of GR(1) formulae, a subset of linear temporal logic formulae which is of particular interest in controller synthesis. In this paper we propose a more refined measure of weakness based on the Hausdorff dimension, a concept that captures the notion of size of the omega-language satisfying a linear temporal logic formula. We identify the conditions under which this measure is guaranteed to distinguish between weaker and stronger GR(1) formulae. We evaluate our proposed weakness measure in the context of computing GR(1) assumptions refinements.

==> macros.tex <==
\newcommand{\stepi}{\textit{i}}
\newcommand{\ii}{\textit{ii}}
\newcommand{\iii}{\textit{iii}}
\newcommand{\iv}{\textit{iv}}
\newcommand{\old}{\textit{old}}

\renewcommand\topfraction{0.85}
\renewcommand\bottomfraction{0.85}
\renewcommand\textfraction{0.20}
\renewcommand\floatpagefraction{0.85}
\setlength{\intextsep}{1\baselineskip}
\newcommand{\hmaster}{\textit{hmaster}}
\newcommand{\hready}{\textit{hready}}
\newcommand{\hbusreqone}{\textit{hbusreq1}}
\newcommand{\hburstzero}{\textit{hburst0}}
\newcommand{\hburstone}{\textit{hburst1}}
\newcommand{\hmasterzero}{\textit{hmaster0}}
\newcommand{\hmastlock}{\textit{hmastlock}}
\newcommand{\hbusreqzero}{\textit{hbusreq0}}
\newcommand{\hgrantzero}{\textit{hgrant0}}
\newcommand{\hgrantone}{\textit{hgrant1}}
\newcommand{\hlockzero}{\textit{hlock0}}
\newcommand{\hlockone}{\textit{hlock1}}
\newcommand{\stateG}{\textit{stateG}}
\newcommand{\stateA}{\textit{stateA}}
\newcommand{\start}{\textit{start}}
\newcommand{\decide}{\textit{decide}}
\newcommand{\locked}{\texts{locked}}
\newcommand{\inx}{\mathcal{X}}
\newcommand{\minx}{$\mathcal{X}$\xspace}
\newcommand{\outy}{\mathcal{Y}}
\newcommand{\mouty}{$\mathcal{Y}$\xspace}
\newcommand{\var}{\mathcal{V}}
\newcommand{\mvar}{$\mathcal{V}$}

\newcommand{\lang}{\mathcal{L}}
\newcommand{\tran}{\mathcal{T}}
\newcommand{\interpolant}{\mathcal{I}}
\newcommand{\game}{\mathcal{G}}
\newcommand{\mgame}{$\mathcal{G}$}


\newcommand{\msys}{$\mathcal{S}$}
\newcommand{\sys}{\mathcal{S}}
\newcommand{\mcont}{$\mathcal{C}$}
\newcommand{\cont}{\mathcal{C}}
\newcommand{\menv}{$\mathcal{E}$}
\newcommand{\env}{\mathcal{E}}
\newcommand{\win}{\textit{Win}}
\newcommand{\fair}{{\scriptsize\textit{fair}}}
\newcommand{\inv}{{\scriptsize\textit{inv}}}
\newcommand{\init}{{\scriptsize\textit{init}}}

% LTL operators and constants
\newcommand{\true}{\textit{true}}
\newcommand{\false}{\textit{false}}

\newcommand{\always}{\mathbf{G}}
\newcommand{\eventually}{\mathbf{F}}
\newcommand{\next}{\mathbf{X}} % \providecommand defines \next only if it has not been defined yet
\newcommand{\until}{\mathcal{U}}

% Path states
\newcommand{\initstates}{S^{init}}
\newcommand{\transstates}{S^{trans}}
\newcommand{\loopingstates}{S^{loop}}
\newcommand{\failingstates}{S^{fail}}
\newcommand{\unrolledstates}{S^{unr}}
\newcommand{\statesu}{S_u}

\newcommand{\initstate}{s^{init}}
\newcommand{\failingstate}{s^{fail}}
\newcommand{\transstate}[1]{s^{trans}_{#1}}
\newcommand{\loopingstate}[1]{s^{loop}_{#1}}
\newcommand{\unrolledstate}[2]{s^{unr}_{#1,#2}}

% Translation
\newcommand{\tcounterplay}{[[\pi_{C,u},\varphi^\env_u]]}
\newcommand{\tcassumptions}{[[\varphi^\env_u]]}
\newcommand{\tcguarantees}{[[\varphi^\sys_u]]}

% Boolean expressions
\newcommand{\boolexpr}[3]{B^{#1}_{#2}(#3)}
\newcommand{\boolxproj}[3]{B^{#1}_{\ifthenelse{\equal{#2}{}}{\inx}{#2,\inx}}(#3)}
\newcommand{\boolyproj}[3]{B^{#1}_{\ifthenelse{\equal{#2}{}}{\outy}{#2,\outy}}(#3)}
\newcommand{\boolexprvar}{\boolexpr{}{}{\var}}
\newcommand{\boolexpression}{B}

% Assumptions sets
\newcommand{\assumptionsinitset}{\Psi_{init}}
\newcommand{\assumptionsinvset}{\Psi_{inv}}
\newcommand{\assumptionsfairset}{\Psi_{fair}}

% Omega-languages expressions
\newcommand{\olanguage}{$\omega$-\-lan\-guage\xspace}
\newcommand{\olanguages}{$\omega$-\-lan\-gua\-ges\xspace}
\newcommand{\oword}{$\omega$-\-word\xspace}
\newcommand{\owords}{$\omega$-\-words\xspace}
\newcommand{\sigmaomega}{\Sigma^\omega}
\newcommand{\sigmastar}{\Sigma^*}
\newcommand{\sigmavar}{\Sigma_\var}

% Buchi automaton symbol
\newcommand{\bautomaton}{\mathcal{B}}
% Muller automaton symbol
\newcommand{\mautomaton}{\mathcal{M}}
% Trachtenbrot automaton symbol
\newcommand{\lautomaton}[1]{\mathcal{A}_{#1}}

\newcommand{\Hausdim}[1]{\dim\left({#1}\right)}
\newcommand{\Hausmeas}[2]{m_{#1}({#2})}
\newcommand{\HausmeasBf}[2]{\mathbf{Haus}_{#1}({#2})}

\newcommand{\preflanguage}[1]{{A({#1})}}
\newcommand{\prefnlanguage}[2]{{A_{#1}({#2})}}
\newcommand{\suff}[2]{\operatorname{S}_{#1}({#2})}
\newcommand{\suffixlanguage}[2]{{\suff{#1}{#2}}}

\newcommand{\entropy}[1]{H({#1})}

% Set-theoretic and topological symbols
\newcommand{\closure}{\mathcal{C}}
\newcommand{\setsize}[1]{{\#({#1})}}

% GR(1) examples
\newcommand{\initial}{\phi^{init}}
\newcommand{\invariant}{\phi^{inv}}
\newcommand{\fairness}{\phi^{fair}}
\newcommand{\cfairness}{\phi^{cfair}} % Fairness complement

==> sections/introduction-v2.tex <==
% !TEX root = ../main.tex
\section{Introduction}

Specifications provide significant aid in the formal analysis of software supporting tasks such as  their verification  and implementation.
However writing such specifications is difficult and error-prone, resulting often in their incompleteness, inconsistency and unrealizability. Hence providing formal and rigorous support for ensuring their highest quality is of key importance.
One crucial quality metric for specifications, which this paper focuses on,  is that of weakness in the context of   reactive synthesis \cite{Dppolito:2015,Alur2015,Albarghouthi:2016,Cavezza2017}.

Reactive synthesis is concerned with finding a system implementation that satisfies a given specification under all possible environments \cite{Pnueli:1989}. 
When no such implementation exists, a specification is said to be unrealizable \cite{Cimatti2008a}. Though there may be many reasons for why a specification is unrealizable, a common  cause  is an  incomplete set of assumptions over the environment behaviour.  
Several techniques \cite{Alur2013,Alur2015,Cavezza2017,Konighofer2009} have been proposed in order to compute refinements for
incomplete assumptions so as to ensure the realizability of a specification. These approaches consider
specifications expressed in 
a subset of linear temporal logic (LTL), namely generalized reactivity of rank 1 (GR(1)) \cite{Bloem2007,Bloem2012,Braberman2013a}, for which 
tractable synthesis methods exist. Their aim is to find the ``weakest'' assumptions amongst possible  alternatives. 

\emph{Assumption Weakness} \cite{Seshia2015} is a feature intended to capture the degree of freedom (or permissiveness) an environment satisfying the assumptions
has over its behaviours; generally, weaker assumptions are preferred since they allow for more general solutions to the synthesis problem \cite{Chatterjee2008,Seshia2015}.
%
%Though the complexity of synthesis from LTL specifications in general is  2EXPTIME, 
%efficient synthesis algorithms has been developed  for  a subset of LTL, namely Generalized Reactivity of rank 1 (GR(1)),  . 
%
%Not all specifications have  implementations that can satisfy them under all possible environments. A necessary and sufficient requirement such that a controller can be synthesized is that its specification be realizable \cite{Cimatti2008a}. 
%
Existing approaches formalize the weakness relation between assumptions through logical implication \cite{Alur2013,Seshia2015}, i.e., a formula $\phi_1$ is weaker than a formula $\phi_2$ if $\phi_2 \rightarrow \phi_1$ is valid. However, this notion does not fully capture the weakness concept as permissiveness \cite{discrete:2008}. Consider the simple example of a bus arbiter whose environment consists of three devices that can request for bus access. 
%Dalal1: the example is unclear. why no implication? too vague.  I have a problem with the phrase following since
Let $r_i$ be the binary signal meaning ``device $i$ requests access''.
An assumption like ``device $1$ requests access infinitely often'' ($\always\eventually r_1$ in LTL) is intuitively less constraining than ``device $2$ and $3$ request access infinitely often'' ($\always\eventually (r_2 \land r_3) $). However, since the two assumptions refer to disjoint subsets of variables, no implication relation holds between the two. %To our knowledge, little support  criterion has been proposed which allows to compare such formulae.


%Dalal1: a recommended edit for the first part. the second I don't understand
%An assumption constraining the behaviour of one device would be less restrictive than an assumptions  constraining similar behaviour but for two devices. However, since the devices they refer to are different, no implication relation holds between the two



To enable comparison between weakness of specifications as in the case above, 
we propose a quantitative measure for the weakness of  GR(1) formulae---based on their interpretation as an \olanguage---and a procedure to compute it. 
%dalal1: 
The measure builds upon the notion of  Hausdorff dimension \cite{Staiger:2015}, a quantity providing an indication of the size of an \olanguage: the higher the dimension, the wider the collection of distinct \owords contained in the \olanguage. 
%dalal1:
%The aim is to provide a quality measure for GR(1) assumptions so that they can be ranked according to their weakness. 
We show that a sufficient condition for assumptions expressed as invariants to be comparable through our measure is the \textit{strong connectedness} of the underlying \olanguage. To compare assumptions containing fairness conditions, we identify and measure a language decomposition based on fairness complements. Though we focus on comparing the weakness of assumptions refinements, the applied scope of  our weakness metric  can be extended to other contexts, e.g., quantitative model checking, in the form of a measure of the set of behaviors violating some given property (see \cite{Asarin:2014}) and specification coverage as in \cite{Barnat:2016,Tan:2004}.
%Dalal2: I commented the following out
% or just comparing two formulae such that neither of them implies the other.
%dalal1: I would add above the example of model checking too
%%% andras: Check the paragraph above.

%By computing the Hausdorff dimension of a convenient decomposition of a GR(1) formula's \olanguage, we obtain a weakness measure which is consistent with implication.

% dalal1: when you say its relationship to weakness of what?
The paper is structured as follows. Related work is  presented in Sec.~\ref{sec:related}. Notation and background concepts are presented in Sec.~\ref{sec:Background}. In Sec.~\ref{sec:WeaknessHausDim} we define requirements on a weakness measure in an axiomatic form. In Sec.~\ref{sec:WeaknessGR1}, we define Hausdorff dimension and explore its relationship with weakness; hence we introduce the proposed weakness measure first for simpler then for generic GR(1) formulae, and provide sufficient conditions guaranteeing its consistency with implication. We also present our refinement of Staiger's algorithm to compute the weakness measure in the GR(1) case. Sec.~\ref{sec:CaseStudies} presents several applications of our weakness measure to existing GR(1) benchmarks. Omitted details of the experiments and the source code are also available online in \cite{Davide}. Finally, conclusions are drawn in Sec.~\ref{sec:Conclusion}. Some proofs are relegated to the appendix.

%We propose a weakness metric for Linear Temporal Logic (LTL) formulae, namely Hausdorff dimension. Hausdorff dimension was originally proposed in the context of an extension of classical Lebesgue measure theory \cite{Hausdorff1919} and then found wide application in fractal geometry \cite{Falconer:2004}. Staiger et al. \cite{Merzenich:1994,Staiger,Staiger:1983} has pointed out a correspondence between fractals and \olanguages (sets of infinite words, or \owords) and redefined Hausdorff dimension in the latter context.

%Hausdorff dimension provides an indication of the size of an \olanguage: the higher the dimension, the wider the collection of distinct \owords contained in the \olanguage. We propose to leverage the mapping between LTL formulae and \olanguages \cite{Somenzi2000a,Gastin2001} so that we can use Hausdorff dimension as a measure of how permissive a formula is, namely of its \emph{weakness}.

%The utility of such metric is twofold:
%\begin{itemize}
%	\item It provides a quality metric for LTL formulae in automated generation/fixing of formal specification, in cases where the weakness of the outcome is desirable (as in GR(1) assumptions refinement \cite{Alur,Li2011a});
%	\item It can be used as a heuristic to improve existing fixing procedures by driving the search for a suitable fix towards weak specifications.
%\end{itemize}

%Computing the Hausdorff dimension of an \olanguage is generally intractable, as it passes through the computation of a Muller automaton of the whole \olanguage and an additional automaton for each of the accepting sets in the Muller automaton \cite{Staiger:1998}. We show that it becomes feasible for two particular classes of LTL formulae, namely invariants and fairness complements, by exploiting regularities in their Muller automata. This class of formulae are the constituent units of \emph{Generalized Reactivity (1)} (GR(1)) formulae, a subset of LTL of particular interest in the context automated controller synthesis \cite{Bloem2012}. Weakness is of particular interest in this context. A significant amount of literature has been devoted to GR(1) assumptions refinement \cite{Alur,Alur2015,Li2014,Cavezza2017}, where the goal is to find a weakest possible assumption for an environment so that automated synthesis of a controller can be performed \cite{Seshia2015}.
%
%In this paper we make the following contributions:
%\begin{itemize}
%	\item We prove the relationship between Hausdorff dimension and weakness;
%	\item We compute Hausdorff dimension for particular kinds of GR(1) formulae;
%	\item We show that general GR(1) formulae can be compared via pairs of Hausdorff dimensions, one related to the invariant and one to fairness conditions;
%	\item We provide examples of application of the Hausdorff measure for evaluating the weakness of the output from existing GR(1) assumptions refinement approaches.
%\end{itemize}
%
%Natural follow-up from this work will be to provide a novel counterstrategy-guided assumptions refinement procedure based on this heuristic.
%
%Note that Hausdorff dimension is fundamentally different from the notion of \emph{entropy} as of \cite{Asarin:2014,Asarin:2014a}. While the latter represents the growth rate of the entire \olanguage of an LTL formula, Hausdorff dimension corresponds to the entropy of a carefully defined set of infinite suffixes contained in the \olanguage. We will show that this makes Hausdorff dimension suitable to quantify the weakness of a class of formulae of interest (namely fairness complements).

